Analysis of the decay $D^0\rightarrow K_{S}^{0} K^{+} K^{-}$

Using a data sample of $2.93~fb^{-1}$ of $e^+e^-$ collisions collected at $\sqrt{s}=3.773 GeV$ in the BESIII experiment, we perform an analysis of the decay $D^0\rightarrow K_{S}^{0} K^{+} K^{-}$. The Dalitz plot is analyzed using $1856\pm 45$ flavor-tagged signal decays. We find that the Dalitz plot is well described by a set of six resonances: $a_0(980)^0$, $a_0(980)^+$, $\phi(1020)$, $a_2(1320)^+$, $a_2(1320)^-$ and $a_0(1450)^-$. Their magnitudes, phases and fit fractions are determined as well as the coupling of $a_0(980)$ to $K\bar{K}$, $g_{K\bar{K}}=3.77\pm 0.24\text{(stat.)}\pm0.35\text{(sys.)} GeV$. The branching fraction of the decay $D^0\rightarrow K_{S}^{0} K^{+} K^{-}$ is measured using $11660\pm 118$ untagged signal decays to be $(4.51\pm 0.05\text{(stat.)}\pm 0.16\text{(sys.)})10^{-3}$. Both measurements are limited by their systematic uncertainties.

==> alias.tex <==
\RequirePackage{xspace}


\newcommand{\ie}{i.\,e.\xspace}
\newcommand{\Ie}{I.\,e.\xspace}
\newcommand{\eg}{e.\,g.\xspace}
\newcommand{\Eg}{E.\,g.\xspace} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% DEPRECATED %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\GeV}{\si{\giga\electronvolt}\xspace}
\newcommand{\MeV}{\si{\mega\electronvolt}\xspace}
\newcommand{\KeV}{\si{\kilo\electronvolt}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% EXPERIMENTS %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\textbf\sl B}\hspace{-0.1em}{\LARGE\textbf\sl A}\hspace{-0.03em}{\huge\textbf\sl B}\hspace{-0.1em}{\LARGE\textbf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}

\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}\xspace}
\def\pep2{PEP-II}
\newcommand{\panda}{PANDA\xspace}
\newcommand{\bes}{\mbox{BESIII}\xspace}
\newcommand{\besSc}{\fontfamily{ppl}\selectfont\textsc{Besiii}\normalfont\xspace}
\newcommand{\lhcb}{LHCb\xspace}
\newcommand{\cleo}{\textsc{Cleo}\xspace}
\newcommand{\cleoc}{\cleo-c\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% SOME DEFS %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\particle}[1]{{\ensuremath{\mathrm #1}}\xspace}
%\newcommand{\BAR}[1]{\overline{#1}}
\newcommand{\BAR}[1]{\kern 0.2em\overline{\kern -0.2em #1}{}\xspace}
%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%overline for normal text
\makeatletter
\newcommand*{\textover}[1]{\ensuremath{\overline{\hbox{#1}}\m@th}}
\makeatother

%\newcommand{\sgn}{\mathop{\mathrm{sgn}}} %sign operator; requires amsmath
\DeclareMathOperator{\sgn}{sgn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
%\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\mathrm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\KKbar {\ensuremath{\kaon\Kbar}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
%\def\KK    {\ensuremath{\KpKm}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\DD      {\ensuremath{D\Dbar}\xspace} 
\def\DDbar   {\DD\xspace}
\def\D       {\ensuremath{D}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\kern 0.2em\overline{\kern -0.2em D}\rule{0pt}{1.5ex}{}^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% QUARKONIA %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\psipp 	  {\psiprpr}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\p      	 {\proton\xspace}
\def\pbar      	 {\antiproton\xspace}
\def\ppbar       {\proton\antiproton\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}
\def\n 			 {\neutron\xspace}
\def\nbar 		 {\antineutron\xspace}
\def\nnbar 		 {\neutron\antineutron\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\mathcal B}}\xspace}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{\ensuremath{p}}\xspace}
\def\pt         {\mbox{\ensuremath{p_T}}\xspace}
\def\mes        {\mbox{\ensuremath{m_{\mathrm ES}}}\xspace}
\def\mec        {\mbox{\ensuremath{m_{\mathrm EC}}}\xspace}
\def\DeltaE     {\mbox{\ensuremath{\Delta E}}\xspace}
\def\qsq        {\ensuremath{q^2}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{\ensuremath{\phi}}\xspace}
\def\mtheta     {\mbox{\ensuremath{\theta}}\xspace}
\def\ctheta     {\mbox{\ensuremath{\cos\theta}}\xspace}
\def\cosTheta 	{\ensuremath{\cos(\Theta)}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   UNITS   %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareSIUnit\c{c}
\DeclareSIUnit\cSq{\c^2}
\DeclareSIUnit\eV{\tera\electronvolt}
\DeclareSIUnit\eVc{\electronvolt/\c}
\DeclareSIUnit\eVcSq{\electronvolt/\cSq}
\DeclareSIUnit\KeV{\kilo\electronvolt}
\DeclareSIUnit\MeV{\mega\electronvolt}
\DeclareSIUnit\GeV{\giga\electronvolt}
\DeclareSIUnit\TeV{\tera\electronvolt}
\DeclareSIUnit\invfb{\femto\barn\tothe{-1}}
\DeclareSIUnit\invpb{\pico\barn\tothe{-1}}
\DeclareSIUnit\timesten{\ensuremath{\times}10}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Some more (from Helen)
%\def\O{{\ensuremath{\mathcal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\mathcal O}}\xspace}
\def\L{{\ensuremath{\mathcal L}}\xspace}
\def\mathcalL{{\ensuremath{\mathcal L}}\xspace}
%\def\S{{\ensuremath{\mathcal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\mathcalS{{\ensuremath{\mathcal S}}\xspace}
\def\mathcalA{{\ensuremath{\mathcal A}}\xspace}
\def\mathcalD{{\ensuremath{\mathcal D}}\xspace}
\def\mathcalR{{\ensuremath{\mathcal R}}\xspace}

\def\jmathBar{{\ensuremath{\overline{\jmath}}}\xspace}
\def\imathBar{{\ensuremath{\overline{\jmath}}}\xspace}


\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

% Data processing
\def\kbytes     {\ensuremath{{\mathrm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\mathrm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\mathrm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\mathrm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\mathrm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\mathrm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\mathrm \,Tbytes/yr}}\xspace}

% QCD parameters
\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters
\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation
\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
\def\CPV                {\ensuremath{C\!P\!V}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\G       {\ensuremath{G}\xspace}
\def\T       {\ensuremath{T}\xspace}
\def\JPC       {\ensuremath{J^{\P\C}}\xspace}
\def\JP       {\ensuremath{J^{\P}}\xspace}
\def\IG       {\ensuremath{I^{\G}}\xspace}

\def\epstag  {\ensuremath{\varepsilon_{\mathrm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\mathcal D}\xspace}
\def\deltaz{\ensuremath{{\mathrm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\mathrm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\mathrm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}
\newcommand{\qcd}{\ensuremath{\mathrm{QCD}}\xspace}
\newcommand{\QED}{\ensuremath{\mathrm{QED}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
%\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
%\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
%\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
%\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
%\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.\xspace}
% update the following based on input from John Ripka, Asst. Editor at PRL, August 2006
\newcommand{\nimBaseA}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ A\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ B\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ C\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ D\xspace}
\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ E\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\textbf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\textbf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\textbf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\textbf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\textbf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\textbf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\textbf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\textbf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\textbf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\textbf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\textbf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\textbf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\textbf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\textbf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\textbf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\textbf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\textbf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\textbf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\textbf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\textbf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\textbf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\textbf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\textbf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\textbf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\textbf A{\textbf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\textbf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\textbf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\textbf G{\textbf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\textbf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\textbf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\textbf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\textbf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\textbf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\textbf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\textbf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\textbf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\textbf A{\textbf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~{\textbf #1}}
\newcommand{\nimb}      [1]  {\nimBaseB~{\textbf #1}}
\newcommand{\nimc}      [1]  {\nimBaseC~{\textbf #1}}
\newcommand{\nimd}      [1]  {\nimBaseD~{\textbf #1}}
\newcommand{\nime}      [1]  {\nimBaseE~{\textbf #1}}
% add commands for NIM articles from earlier periods
% for NIM articles from 1981-1983
\newcommand{\oldnim}    [1]  {Nucl.\ Instrum.\ Methods Phys.\ Res.~{\textbf #1}}
% for NIM articles prior to 1981
\newcommand{\oldernim}  [1]  {Nucl.\ Instrum.\ Methods~{\textbf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\textbf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\textbf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\textbf B{\textbf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\textbf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\textbf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\textbf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\textbf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\textbf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\textbf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\textbf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\textbf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\textbf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\textbf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\textbf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\textbf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\textbf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\textbf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\textbf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\textbf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\textbf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\textbf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\textbf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\textbf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\textbf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\textbf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\textbf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\textbf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\textbf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\textbf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\textbf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\textbf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\textbf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\textbf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\textbf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\textbf #1}}}
\newcommand{\sci}       [1]  {{Science~{\textbf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\textbf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\textbf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\textbf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\textbf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\textbf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\textbf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\textbf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\textbf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\textbf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\textbf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sftName}[1]{\mbox{\textsc{#1}}\xspace} %
\def\aslund     {\sftName{Aslund}}
\def\bbsim      {\sftName{BBsim}}
\def\beast      {\sftName{Beast}}
\def\beget      {\sftName{Beget}}
\def\Bta        {\sftName{Beta}}
\def\betakfit   {\sftName{BetaKfit}}
\def\cornelius  {\sftName{Cornelius}}
\def\evtgen     {\sftName{EvtGen}}
\def\euclid     {\sftName{Euclid}}
\def\fitver     {\sftName{FitVer}}
\def\fluka      {\sftName{Fluka}}
\def\fortran    {\sftName{Fortran}}
\def\gcalor     {\sftName{GCalor}}
\def\geant      {\sftName{GEANT}}
\def\gheisha    {\sftName{Gheisha}}
\def\hemicosm   {\sftName{HemiCosm}}
\def\hepevt     {\sftName{HepEvt}}
\def\jetset74   {\sftName{Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\sftName{KoralB}}
\def\minuit     {\sftName{Minuit}}
\def\objegs     {\sftName{Objegs}}
\def\paw        {\sftName{Paw}}
\def\Root       {\sftName{Root}}
\def\squaw      {\sftName{Squaw}}
\def\stdhep     {\sftName{StdHep}}
\def\trackerr   {\sftName{TrackErr}}
\def\turtle     {\sftName{Decay~Turtle}}
\providecommand{\mLyX}{L\kern-.1667em\lower.25em\hbox{Y}\kern-.125emX\@}
\def\COMPWA {\sftName{ComPWA}}
\def\MINUIT {\sftName{Minuit}}
\def\MIGRAD {\sftName{Migrad}}
\def\MINOS 	{\sftName{Minos}}
\def\HESSE  {\sftName{Hesse}}
\def\Minuit {\sftName{Minuit}}
\def\Migrad {\sftName{Migrad}}
\def\Minos  {\sftName{Minos}}
\def\Hesse  {\sftName{Hesse}}
\def\BOSS   {\sftName{BOSS}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own aliases
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\DKsKK}{\ensuremath{\Dz\to\KsKK}\xspace}
\newcommand{\KsKK}{\ensuremath{\KS\KpKm}\xspace}
\newcommand{\Kppim}{\ensuremath{\Kp\kern -0.16em \pim}\xspace}
\newcommand{\pipiKK}{\ensuremath{\pipi\kern -0.16em\KpKm}\xspace}
\newcommand{\dtagZero}{\ensuremath{K^-\pi^+}\xspace}
\newcommand{\dtagOne}{\ensuremath{K^-\pi^+\pi^0}\xspace}
\newcommand{\dtagThree}{\ensuremath{K^-\pi^+\pi^-\pi^+}\xspace}
\newcommand{\bkgOne}{\ensuremath{\text{Bkg}_{\text{KS}}}\xspace}
\newcommand{\bkgTwo}{\ensuremath{\text{Bkg}_{\text{nonKS}}}\xspace}
\newcommand{\phiPiPi}{\ensuremath{\Dz\to(KK)_{\phi}(\pi\pi)_\rho}\xspace}

\newcommand{\Amp}{\ensuremath{{\mathcal M}}\xspace}
\newcommand{\lumi}{\ensuremath{{\mathcal L}}\xspace}
\newcommand{\FitPar}{\ensuremath{\boldsymbol\beta}\xspace}
\newcommand{\DPvar}{\ensuremath{\boldsymbol\xi}\xspace}
\newcommand{\mBC}{\ensuremath{m_{bc}}\xspace}
\newcommand{\mKS}{\ensuremath{m_{ks}}\xspace}
\newcommand{\mKK}{\ensuremath{m_{KK}}\xspace}
\newcommand{\helKK}{\ensuremath{\cos\theta_{KK}}\xspace}
\newcommand{\mKSKplus}{\ensuremath{m_{K^0K^+}}\xspace}
\newcommand{\mKSKminus}{\ensuremath{m_{K^0K^-}}\xspace}
\newcommand{\mKKsq}{\ensuremath{\mKK^{2}}\xspace}
\newcommand{\mKSKplusSq}{\ensuremath{\mKSKplus^{2}}\xspace}
\newcommand{\mKSKminusSq}{\ensuremath{\mKSKminus^{2}}\xspace}
\newcommand{\helicityTheta}{\ensuremath{\Theta_{KK}}\xspace}
\newcommand{\FLATTE}{Flatt\'{e}\xspace}

\newcommand{\pull}{\ensuremath{{\mathcal P}}\xspace}
\newcommand{\pValue}{\ensuremath{{\mathcal P}}\xspace}
\newcommand{\prob}{\ensuremath{{\mathcal P}}\xspace}
\newcommand{\likelih}{\ensuremath{{\mathcal L}}\xspace}


==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_PROGRAM_AUTHOR	Darren Hiebert	/dhiebert@users.sourceforge.net/
!_TAG_PROGRAM_NAME	Exuberant Ctags	//
!_TAG_PROGRAM_URL	http://ctags.sourceforge.net	/official site/
!_TAG_PROGRAM_VERSION	5.8	//
#1	templates/sample/aps/apssamp.tex	/^\\verb+\\section{#1}+ the \\verb+#1+ stands for the title text of the$/;"	s
A few notes on texttt tag	templates/sample/aps/apssamp.tex	/^\\end{equation}$/;"	P
A little more on appendixes	templates/sample/aps/apssamp.tex	/^\\begin{verbatim}$/;"	s
A little more on appendixes	templates/sample/aps/apssamp.tex	/^command (\\verb+\\appendix*+ in the place of \\verb+\\appendix+).$/;"	s
Abstract	templates/aps/apsguide4-1.tex	/^\\end{itemize}$/;"	b
Acknowledgments	acknowledgements.tex	/^\\section{Acknowledgments}$/;"	s
Appendixes	templates/sample/aps/apssamp.tex	/^\\appendix$/;"	s
Authors affiliations and collaborations	templates/aps/apsguide4-1.tex	/^title.$/;"	b
Background	AmplitudeAnalysis.tex	/^The Dalitz plot analysis is performed using the \\sftName{ComPWA} framework~\\cite{Michel:2014nza, ComPWA:DKsKK}.$/;"	b
Background	templates/sample/aps/apssamp.tex	/^\\appendix$/;"	s
Bold symbols in math	templates/auguide/auguide4-1.tex	/^documentation for the complete list of symbols available.$/;"	b
Branching fraction measurement	BF.tex	/^\\section{Branching fraction measurement}$/;"	s
Bug Fixes in revtex 4 1	templates/auguide/whatsnew4-1.tex	/^\\end{itemize}$/;"	s
Changes in revtex 4 1	templates/auguide/auguide4-1.tex	/^distribution.$/;"	b
Citations and References	templates/aip/aipguide4-1.tex	/^footnotes may be incorporated into text during the production process.$/;"	s
Citing a reference	templates/auguide/auguide4-1.tex	/^particular the \\verb+natnotes.tex+ file for a convenient summary. Please also note that \\classname{natbib 8.3} and later now gives an error (rather than merely a warning as in earlier versions) if you try to use a Bib\\TeX\\ file that isn't compatible with author-year style citations with a journal style that requires author-year citations (such as \\textit{Reviews of Modern Physics}).$/;"	b
Combined Author Year and Numeric Citations	templates/auguide/auguide4-1.tex	/^guidelines regarding \\classname{natbib}'s macros.$/;"	b
Comments from Hailong	Answers.tex	/^\\begin{document}$/;"	s
Comments from Hajime	Answers.tex	/^\\end{enumerate}$/;"	s
Comments from Shuangshi	Answers.tex	/^\\end{enumerate}$/;"	s
Conclusion	Conclusion.tex	/^\\section{Conclusion}$/;"	s
Cross referencing	templates/sample/aip/aipsamp.tex	/^this paragraph, there is no paragraph indent for this paragraph.)$/;"	s
Cross referencing	templates/sample/aps/apssamp.tex	/^and the start of this paragraph, this paragraph is not indented.)$/;"	s
Dalitz plot analysis	AmplitudeAnalysis.tex	/^\\section{Dalitz plot analysis}$/;"	s
Data preparation	Selection.tex	/^\\section{Data preparation}$/;"	s
Detection and data sets	DetectorData.tex	/^\\section{Detection and data sets}$/;"	s
Event selection	Selection.tex	/^\\label{sec:dataPrep}$/;"	b
Example references	templates/sample/aps/apssamp.tex	/^respectively. To display titles for cited journal articles, use the \\texttt{longbibliography} class option.$/;"	b
Figures and Artwork	templates/auguide/auguide4-1.tex	/^Please note the use of curly braces to enclose the text within the square brackets as well as the spaces next to the brackets.$/;"	s
Figures and Tables	templates/sample/aip/aipsamp.tex	/^and Fig.~\\ref{fig:epsart}.$/;"	s
Floats Figures Tables Videos etc	templates/sample/aps/apssamp.tex	/^\\end{figure}$/;"	s
Fonts	templates/auguide/auguide4-1.tex	/^\\LaTeXe\\ markup is the preferred way to accomplish many basic tasks.$/;"	b
Footnotes	templates/aip/aipguide4-1.tex	/^Herein are some features specific to the AIP author.$/;"	b
Footnotes	templates/auguide/auguide4-1.tex	/^preceded by \\cmd\\protect\\ in commands with moving arguments.$/;"	s
Footnotes	templates/sample/aps/apssamp.tex	/^and compare its information to the formatted bibliography itself.$/;"	b
Footnotes for authors collaborations affiliations or title	templates/auguide/auguide4-1.tex	/^\\cmd\\collaboration\\ with \\cmd\\noaffiliation.$/;"	b
Fourth level heading is run in	templates/sample/aip/aipsamp.tex	/^\\verb+thebibiliography+ environment should be used instead.$/;"	P
Goodness of fit	AmplitudeAnalysis.tex	/^The final model consists of $a_0(980)^0$, $\\phi(1020)$, $a_0(980)^+$, $a_2(1320)^+$, $a_2(1320)^-$ and $a_0(1450)^-$. We rerun the minimization using this model without the penalty term to obtain the final values and uncertainties.$/;"	b
Institutional report numbers	templates/auguide/auguide4-1.tex	/^included in the \\cmd\\documentclass\\ line to display the keywords.$/;"	b
Introduction	templates/aps/apsguide4-1.tex	/^\\tableofcontents$/;"	s
Introduction	templates/auguide/auguide4-1.tex	/^\\begin{verbatim}$/;"	s
Journal Substyle	templates/aip/aipguide4-1.tex	/^\\section{\\revtex\\ Class Options Specific to AIP}$/;"	b
Keywords	templates/auguide/auguide4-1.tex	/^explicitly included in the class options to display the PACS codes.$/;"	b
Likelihood function	AmplitudeAnalysis.tex	/^We insert ${\\mathcal A}(\\FitPar,\\DPvar)$ into ${\\mathcal M}(\\FitPar,\\DPvar)$ (\\cref{eqn:dalitz:qc:DTMatrixEl}) to obtain the decay amplitude including the effect of the quantum entanglement of \\Dz and \\Dzb. $/;"	b
Loading other packages	templates/auguide/auguide4-1.tex	/^and Options Summary}.$/;"	b
Marking up front matter	templates/aps/apsguide4-1.tex	/^be trouble free for all referees.$/;"	s
Multiple references in a single bibliography entry	templates/auguide/whatsnew4-1.tex	/^\\section{\\label{sec:additional}Additional Details}$/;"	b
New Syntax and Features in revtex 4 1	templates/auguide/whatsnew4-1.tex	/^\\maketitle$/;"	s
One column vs two column layouts	templates/auguide/auguide4-1.tex	/^use one or two forward quotes (apostrophes).$/;"	b
Options for Citations and Bibliography	templates/aip/aipguide4-1.tex	/^\\end{table}$/;"	b
PACS codes	templates/auguide/auguide4-1.tex	/^\\end{verbatim}$/;"	b
Paper size	templates/aps/apsguide4-1.tex	/^formatting to single column.$/;"	b
Paragraphs and General Text	templates/auguide/auguide4-1.tex	/^footnotes and \\verb+\\\\+ is a fragile command.)$/;"	b
Placement of Figures Tables and Other Floats	templates/auguide/auguide4-1.tex	/^refer to \\cite{Compan}.$/;"	s
Prepending and or appending text to a citation	templates/auguide/whatsnew4-1.tex	/^One of the most frequently requested features since the release of \\revtex~4 has been to allow more than one reference to appear in a single bibliography entry when using Bib\\TeX. This can now be done in \\revtex~4.1 by using a starred (*) argument to the \\cmd\\cite\\ command. This requires the latest version of \\texttt{natbib}, developed in conjunction with \\revtex~4.1, and the new \\texttt{bst} files that come with \\revtex~4.1. To combine multiple references into a single \\cmd\\bibitem, precede the second, third, etc. citation keys in the \\cmd\\cite\\ command with an asterisk (*). For example \\verb+\\cite{bethe, *feynman, *bohr}+ will combine the \\cmd\\bibitem\\relax s with keys \\texttt{bethe}, \\texttt{feynman}, and \\texttt{bohr} into a single entry in the bibliography separated by semicolons.$/;"	b
Prerequisite Documentation	templates/aip/aipguide4-1.tex	/^except as it bears on the specific features of the AIP substyles.$/;"	b
Quantum entangled texorpdfstring DzDzb	AmplitudeAnalysis.tex	/^\\end{figure}$/;"	b
Quantum entanglement	BF.tex	/^The branching fraction in a single-tag \\DzDzb sample is linked to the branching fraction of an isolated \\Dz decay via the correction factor $f_{QC}$ which is derived in the following.$/;"	b
References	templates/sample/aps/apssamp.tex	/^displays the reference on the baseline.$/;"	b
Resonance model	AmplitudeAnalysis.tex	/^To recap, the result of an analysis of the \\DKsKK Dalitz plot needs to be the amplitude model of an isolated \\Dz decay in order to be comparable with other \\Dz production reactions (\\eg $\\Dstar\\to\\Dz\\pi$). Therefore, we need to incorporate the effect of the decay of a quantum entangled pair of \\Dz mesons as described previously. For many \\Dz final states this effect can be neglected but since \\KsKK is a self-conjugate final state, it needs to be considered.$/;"	b
Resonance selection	Appendix.tex	/^\\section{Resonance selection}$/;"	s
Result	BF.tex	/^The systematic uncertainty, and also the total uncertainty of the measurement is dominated by the contributions due to track reconstruction and particle identification. In total the systematic uncertainty on the branching fraction measurement is \\SI{3.78}{\\percent}.$/;"	b
Sample LaTeXe Document	templates/aip/aipguide4-1.tex	/^if not, it belongs to \\revtex.$/;"	s
Section headings	templates/auguide/auguide4-1.tex	/^following sections carefully. $/;"	b
Setting the title	templates/auguide/auguide4-1.tex	/^different from those provided in the \\LaTeXe\\ \\classname{article} class.$/;"	b
Signal and background	Selection.tex	/^Double-tag and single-tag samples contain \\num{1935(44)} and \\num{13295(115)} candidates, respectively. Contributions to the double-tag sample from individual tag channels are listed in \\cref{tab:sel:tagYields}. The signal yields are determined using a two-dimensional fit to \\mBC and \\mKS.$/;"	b
Software Requirements	templates/aip/aipguide4-1.tex	/^markup guidelines specific to AIP journals. $/;"	b
Some LaTeXe Basics	templates/auguide/auguide4-1.tex	/^sample document that manifests the problem if possible (please don't send large files!). Issues related to the AIP journal styles should be sent directly to \\verb+tex@aip.org+.$/;"	s
Specifying a date	templates/auguide/auguide4-1.tex	/^break in a long title.$/;"	b
Specifying authors and affiliations	templates/auguide/auguide4-1.tex	/^\\end{verbatim}$/;"	b
Specifying first names and surnames	templates/auguide/auguide4-1.tex	/^Please consult the documentation for the various journal style files for further information.$/;"	b
Structured Abstracts	templates/auguide/whatsnew4-1.tex	/^Please note the use of curly braces to enclose the text within the square brackets.$/;"	b
Submitting to AIP Journals	templates/aip/aipguide4-1.tex	/^To obtain the most up-to-date version of this software, please see \\url{http:\/\/www.aip.org\/pubservs\/compuscript.html}.$/;"	b
Submitting to AIP Journals	templates/auguide/auguide4-1.tex	/^Physical Society may be found at \\url{http:\/\/publish.aps.org\/}.$/;"	b
Submitting to APS Journals	templates/auguide/auguide4-1.tex	/^Documents prepared under \\revtex~4 should process correctly under \\revtex~4.1. However, the formatting of the pages and, if using Bib\\TeX, the references may change.$/;"	b
Symbols	templates/auguide/auguide4-1.tex	/^\\textit{APS Author Guide for \\revtex~4.1} when defining macros.$/;"	b
Systematic uncertainties	BF.tex	/^ The quantities $r_j$ and $\\delta_j$ depend on the phase space position and we use the phase space averaged values $\\expval{r_j}$ and $\\expval{\\delta_j}$ for the calculation of $f_{QC}$. From the Dalitz amplitude model a value of $f_{QC} = \\num{2.07(3)}$ is obtained for the final state $j=\\KsKK$. The statistical uncertainty of the Dalitz amplitude model is propagated to $f_{QC}$ via a MC approach. The limited statistics in the double-tag Dalitz plot analysis causes a rather large uncertainty on $f_{QC}$ of \\SI{1.45}{\\percent}.$/;"	b
Tables	templates/auguide/auguide4-1.tex	/^There is also a corresponding \\cmd\\listofvideos\\ command.$/;"	s
The Document Preamble	templates/auguide/auguide4-1.tex	/^\\end{description}$/;"	s
The Front Matter	templates/auguide/auguide4-1.tex	/^\\verb+\\usepackage{graphics}+.$/;"	s
The body of the paper	templates/auguide/auguide4-1.tex	/^explicitly).$/;"	s
The emph documentclass	templates/auguide/auguide4-1.tex	/^load other macro packages, and other macro definitions.$/;"	b
Title	templates/aps/apsguide4-1.tex	/^in the front matter are not needed and should not be used.$/;"	b
Title and Front Matter	templates/aip/aipguide4-1.tex	/^for further details. $/;"	b
Useful LaTeXe Markup	templates/auguide/auguide4-1.tex	/^versions of \\LaTeXe.$/;"	b
User defined macros	templates/auguide/auguide4-1.tex	/^\\end{table}$/;"	b
Using LaTeXe packages with revtex	templates/auguide/auguide4-1.tex	/^\\end{verbatim}$/;"	b
Using protect revtex	templates/00readme.tex	/^\\tableofcontents$/;"	s
Wide equations	templates/sample/aip/aipsamp.tex	/^Eqs.~(\\ref{eq:whole}).$/;"	b
Wide equations	templates/sample/aps/apssamp.tex	/^Eqs.~(\\ref{eq:whole}).$/;"	b
heading	templates/auguide/summary4-1.tex	/^\\verb+\\section*{<heading>}+ & Start a new section without a number.\\\\$/;"	s
heading	templates/auguide/summary4-1.tex	/^\\verb+\\section{<heading>}, \\subsection{<heading>}+,$/;"	b
heading	templates/auguide/summary4-1.tex	/^\\verb+\\section{<heading>}, \\subsection{<heading>}+,$/;"	s
heading	templates/auguide/summary4-1.tex	/^\\verb+\\subsubsection{<heading>}+ & Start a new section or subsection.\\\\$/;"	b
label app subsec	templates/sample/aps/apssamp.tex	/^\\end{equation}$/;"	b
label sec additional	templates/auguide/whatsnew4-1.tex	/^The vast majority of documents prepared under \\revtex~4 should process correctly under \\revtex~4.1. However, the formatting of the pages and, if using Bib\\TeX, the references may change. Also, the behavior of some macros may be different. For instance, the \\texttt{title} macro now requires the use of \\texttt{protect} for fragile arguments. This may cause some documents prepared under \\revtex~4 to fail under 4.1. Some macro packages that depend on the internals of \\revtex~4 may also no longer work.  Documents using those packages will, of course, also will not process under 4.1.$/;"	s
label sec intro	templates/auguide/auguide4-1.tex	/^\\begin{verbatim}$/;"	s
label sec level1	templates/sample/aps/apssamp.tex	/^\\maketitle$/;"	s
label sec level2	templates/sample/aip/aipsamp.tex	/^paragraph has ended. $/;"	b
label sec level3	templates/sample/aip/aipsamp.tex	/^instead.$/;"	b
label sec multiple	templates/auguide/auguide4-1.tex	/^will include the arXiv.org e-print identifier as \\texttt{arXiv:hep-th\/9108028} and hyperlink it (if using \\texttt{hyperref}). The newer format for arXiv identifiers with primary classificiations will produce output such as \\texttt{arXiv:0905.1949 [hep-ph]}.$/;"	b
label sec prepend	templates/auguide/auguide4-1.tex	/^One of the most frequently requested features since the release of \\revtex~4 has been to allow more than one reference to appear in a single bibliography entry when using Bib\\TeX. This can now be done in \\revtex~4.1 by using a starred (*) argument to the \\cmd\\cite\\ command. This requires the latest version of \\texttt{natbib}, developed in conjunction with \\revtex~4.1, and the new \\texttt{bst} files that come with \\revtex~4.1. To combine multiple references into a single \\cmd\\bibitem, precede the second, third, etc. citation keys in the \\cmd\\cite\\ command with an asterisk (*). For example \\verb+\\cite{bethe, *feynman, *bohr}+ will combine the \\cmd\\bibitem\\relax s with keys \\texttt{bethe}, \\texttt{feynman}, and \\texttt{bohr} into a single entry in the bibliography separated by semicolons.$/;"	b
label sec use bib	templates/aip/aipguide4-1.tex	/^There are numerous reasons to use Bib\\TeX, not least because it automates the first and second of the above checks. $/;"	b
label sec use bib	templates/auguide/auguide4-1.tex	/^AIP's \\textit{Journal of Mathematical Physics} uses a combined author\/year and numerical citation style. \\revtex~4.1 supports this referencing style. Please see the \\textit{Author's Guide to AIP Substyles for \\revtex~4.1} for more information about this style.$/;"	b
maketitle	templates/auguide/auguide4-1.tex	/^limited though, so only three or less may actually fit). Please note that the \\classoption{preprint} class option does not automatically invoke \\classoption{preprintnumbers}.$/;"	b
revtex 4 Backwards Compatibility	templates/auguide/auguide4-1.tex	/^\\end{itemize}$/;"	b
revtex 4 Backwards Compatibility	templates/auguide/whatsnew4-1.tex	/^\\end{itemize}$/;"	s
revtex Class Options Specific to AIP	templates/aip/aipguide4-1.tex	/^pertaining to preparing documents under \\LaTeXe\\; they are highly recommended. $/;"	s
texttt figure	templates/auguide/auguide4-1.tex	/^\\section{Figures and Artwork}\\label{sec:figures}$/;"	b
texttt video	templates/auguide/auguide4-1.tex	/^commands inside the float environments.$/;"	b


==> tikzlibrarycustom.code.tex <==
\makeatletter

%------------------------------
%Decent grid with numbered axes
%------------------------------
\def\grd@save@target#1{%
  \def\grd@target{#1}}
\def\grd@save@start#1{%
  \def\grd@start{#1}}
\tikzset{
  grid with coordinates/.style={
    to path={%
      \pgfextra{%
        \edef\grd@@target{(\tikztotarget)}%
        \tikz@scan@one@point\grd@save@target\grd@@target\relax
        \edef\grd@@start{(\tikztostart)}%
        \tikz@scan@one@point\grd@save@start\grd@@start\relax
        \draw[minor help lines] (\tikztostart) grid (\tikztotarget);
        \draw[major help lines] (\tikztostart) grid (\tikztotarget);
        \grd@start
        \pgfmathsetmacro{\grd@xa}{\the\pgf@x/1cm}
        \pgfmathsetmacro{\grd@ya}{\the\pgf@y/1cm}
        \grd@target
        \pgfmathsetmacro{\grd@xb}{\the\pgf@x/1cm}
        \pgfmathsetmacro{\grd@yb}{\the\pgf@y/1cm}
        \pgfmathsetmacro{\grd@xc}{\grd@xa + \pgfkeysvalueof{/tikz/grid with coordinates/major step}}
        \pgfmathsetmacro{\grd@yc}{\grd@ya + \pgfkeysvalueof{/tikz/grid with coordinates/major step}}
        \foreach \x in {\grd@xa,\grd@xc,...,\grd@xb}
        \node[anchor=north] at (\x,\grd@ya) {\pgfmathprintnumber{\x}};
        \foreach \y in {\grd@ya,\grd@yc,...,\grd@yb}
        \node[anchor=east] at (\grd@xa,\y) {\pgfmathprintnumber{\y}};
      }
    }
  },
  minor help lines/.style={
    help lines,
    step=\pgfkeysvalueof{/tikz/grid with coordinates/minor step}
  },
  major help lines/.style={
    help lines,
	line width=\pgfkeysvalueof{/tikz/grid with coordinates/major line width},
    step=\pgfkeysvalueof{/tikz/grid with coordinates/major step}
  },
  grid with coordinates/.cd,
  minor step/.initial=.5,
  major step/.initial=1,
  major line width/.initial=1pt,
}

%------------------------------
% Define styles for the different kind of edges in a Feynman diagram
%------------------------------
\tikzset{
   %eichbosonen
   photon/.style={decorate, decoration={snake}, draw=red},
   wBoson/.style={decorate, decoration={snake}, draw=red},
   zBoson/.style={decorate, decoration={snake}, draw=red},
   gluon/.style={decorate, draw=magenta,decoration={coil,amplitude=2pt, segment length=3pt}},
   %particles
   particle/.style={thin,draw=blue, postaction={decorate},decoration={markings,mark=at position .5 with {\arrow[blue]{stealth}}}},
   electron/.style={draw=blue, postaction={decorate},decoration={markings,mark=at position .55 with {\arrow[draw=blue]{>}}}},
}

\usepackage{environ}
\newsavebox{\measure@tikzpicture}
\NewEnviron{scaletikzpicturetowidth}[1]{%scale tikz pictures to textwidth
   \def\tikz@width{#1}%
   \def\tikzscale{1}\begin{lrbox}{\measure@tikzpicture}%
	  \BODY
   \end{lrbox}%
   \pgfmathparse{#1/\wd\measure@tikzpicture}%
   \edef\tikzscale{\pgfmathresult}%
   \BODY
}
\tikzset{cross/.style={cross out, draw, 
	  minimum size=2*(#1-\pgflinewidth), 
inner sep=0pt, outer sep=0pt}}
\makeatother

